Sparse, Dense, and Attentional Representations for Text Retrieval

Dual encoders perform retrieval by encoding documents and queries into dense lowdimensional vectors, scoring each document by its inner product with the query. We investigate the capacity of this architecture relative to sparse bag-of-words models and attentional neural networks. Using both theoretical and empirical analysis, we establish connections between the encoding dimension, the margin between gold and lower-ranked documents, and the document length, suggesting limitations in the capacity of fixed-length encodings to support precise retrieval of long documents. Building on these insights, we propose a simple neural model that combines the efficiency of dual encoders with some of the expressiveness of more costly attentional architectures, and explore sparse-dense hybrids to capitalize on the precision of sparse retrieval. These models outperform strong alternatives in large-scale retrieval.

==> analyzing_attention.tex <==
\section{Attention}
\label{sec:attention}
Cross attention  involves computations over pairs of tokens, rather than  aggregating texts into single vectors. This requires more computation, but as we show, makes it possible to use much more compact representations than the dual encoder.\footnote{To be precise, we will show that the per-token embedding size can be much smaller for cross attention models; however the entire sequence of tokens is now stored, which is linear in the document length.}
%\kristina{We should be careful to note that the document representation is still growing linearly with the number of tokens as we have more tokens to represent.}
%\jacob{made vaguer}

Let $x = (x_1, x_2, \ldots, x_{\maxtoks_x})$ and  $y = ({y}_{1}, y_2, \ldots, y_{\maxtoks_y}),$ with $x_t, y_t \in \reals^{\embsize}$. (This notation is meant to distinguish between sequence representations and the word count representations $q$ and $d$ from the previous sections.) For example, $x_t$ might represent token $t$ with a contextualized embedding or with an {indicator vector}.
%% cut for space
%, which is zero everywhere except for the position corresponding to token $t$.
The cross attention inner product is defined as,
%%LGTM 
%\kristina{Is this defined in prior work and if so citation?}
%\jacob{I've added some citations that are pretty close to this; they're not super well-known, but the better known papers are not as similar. None explicitly calls it 
%"cross attention inner product", is that a problem?}
%\vspace{-0.6cm}
%\commentout{
\begin{align}
    \psi^{(X)}(x,y) = &{} \sum_{t=1}^{\maxtoks_x} \iprod{x_t}{\sum_{t'=1}^{\maxtoks_y} a_{x,y}(t, t') \times y_{t'}},
\end{align}
\begin{comment}
\begin{align}
    \psi^{(X)}(x,y) = &{} \sum_{t=1}^{\maxtoks_x} \iprod{x_t}{\overline{y}_t}\\
    \overline{y}_t = &{} \sum_{t'=1}^{\maxtoks_y} a_{x,y}(t, t') \times y_{t'},
\end{align}
\commentout{
\begin{equation}
\begin{split}
    & \psi^{(X)}(x,y) =  \sum_{t=1}^{\maxtoks_x} \iprod{x_t} {\overline{y}_t} \\
    &  \overline{y}_t =  \sum_{t'=1}^{\maxtoks_y} a_{x,y}(t, t') \times y_{t'},
\end{split}
\end{equation}
}
\end{comment}
%\vspace{-0.3cm}
where $a_{x,y}(t, t') \in \reals_{+}$ is the attention from token $x_t$ to $y_{t'}$~\cite{yang2016anmm,hao2017end}. 

\begin{definition}
\label{def:hard-attention}
The analysis will focus on \term{normalized hard attention}, which we define as,
\begin{align}
    \tilde{a}_{x,y}(t,t') = &
    \begin{cases}
    1, & \iprod{x_t}{y_t'} > \frac{1}{2}\\
    0, & \text{otherwise}
    \end{cases}\\
    z_{x,y}(t) = &{} \sum_{t'=1}^{\maxtoks_y} \tilde{a}_{x,y}(t,t')\\
    a_{x,y}(t,t') = &{} \tilde{a}_{x,y}(t,t') / z_{x,y}(t), %\sum_{t'=1}^{\maxtoks_y} \tilde{a}_{x,y}(t,t'),
\end{align}
with $0/0 = 0$.
\end{definition}

We now extend the concept of rank preservation  (Definition~\ref{def:rank-preservation}) to token sequences.
\begin{definition}
Let $\set{X}, \set{Y} \subseteq \reals^{\embsize}$ and let $\Count : (\set{X}^* \cup \set{Y}^*) \to \reals^\vocsize$ be an aggregation function\footnote{Here $\set{X}^*$ and $\set{Y}^*$ use Kleene star notation; for example $\set{X}^*$ is the set of all sequences of vectors drawn from $\set{X}$.} such that the inner product $\iprod{\Count(x)}{\Count(y)}$ is a relevance score for the pair $x,y$. A scoring function $\psi: \set{X}^* \times \set{Y}^* \to \reals$ is \term{rank preserving} with respect to $\Count, \set{X}, \set{Y}$ if for all $x, y, y' \in \set{X}^* \times \set{Y}^* \times \set{Y}^*$,
\begin{equation}
%\begin{small}
\begin{split}
    &    (\iprod{\Count(x)}{\Count(y)} > \iprod{\Count(x)}{\Count(y')})\\
&     \Rightarrow (\psi(x,y) > \psi(x,y')).
\end{split}
%\end{small}
\end{equation}
\end{definition}

\newcommand{\indies}[0]{\ensuremath \set{I}}

We next show that cross attention is rank preserving with respect to simple inner product, using indicator vectors and normalized hard attention. For convenience, let $\indies_{\vocsize} = \{ 1_i \}_{i=1}^{\vocsize}$ be the set of indicator vectors over a vocabulary of size $\vocsize$, and define $\Count_{0,1}(x)$ as the vector of elementwise minima $\min(\sum_{t=1}^{\maxtoks_x} x_t, 1),$ so that $\Count_{0,1}(x) \in \{0,1\}^{\vocsize}$ and $\iprod{\Count_{0,1}(x)}{\Count_{0,1}(y)}$ corresponds to simple inner product scoring. The lemma and theorem that follow are restricted to queries without repeated terms, which can be ensured in preprocessing.
\begin{lemma}
For $x \in \indies_{\vocsize}^*$ without repeated terms and for all $y \in \indies_{\vocsize}^*$, the normalized hard attention inner product is identical to the simple inner product, $\psi^{(X)}(x,y) = \iprod{\Count_{0,1}(x)}{\Count_{0,1}(y)}$. 
%% formally: 
% ($\{ x : \max_{i=1\ldots \vocsize} \sum_{t=1}^{\maxtoks_x} x_{t,i} \leq 1\}$). 
\label{lem:hard-attention-is-rank-preserving}
\end{lemma}
\begin{proof}
Space limits permit only a proof sketch. Each $x_t$ has non-zero attention with exactly those $y_{t'}$ such that $\iprod{x_t}{y_{t'}}=1$. There are $z_{x,y}(t)$ such items, and $a_{x,y}(t,t')$ is scaled inversely by this quantity so that $x_t$ contributes exactly $1$ toward the score if it matches any terms in $y$, and zero otherwise. The assumption that there are no repeated terms in $x$ completes the proof.
\end{proof}
\begin{comment}
\begin{remark}
We can make $\psi^{(X)}$ rank preserving with respect to TF-IDF or \bm by scaling the indicator vectors appropriately.
\end{remark}
\end{comment}

\begin{comment}
\begin{definition}
A cross-attention score $\psi^{(X)}(x,y)$ is rank preserving for $x,y,y'$ when,
\begin{equation}
\begin{split}
& \left(\iprod{\sum_t x_t}{\sum_t y_t}
    > \iprod{\sum_t x_t}{\sum_t y'_t}\right)\\
    & \Rightarrow 
    (\psi^{(X)}(x, y) > \psi^{(X)}(x, y')).
    \end{split}
\end{equation}
\end{definition}
\end{comment}

%\subsection{Cross attention and compressive encoding}
%instead that we have compressive encodings of the vocabulary $x_t, y_t \in \reals^{\embsize}$. We now show how to compute an approximate inner product with a compressive encoder.
Let $f$ be a compressive encoder $\indies_{\vocsize} \to \reals^{\embsize}$ with $\embsize < \vocsize$, let $f(x) = (f(x_1), \ldots, f(x_{\maxtoks_x}))$, and define $f(y)$ analogously. This encoder can be viewed as a word embedding function.
Let $\psi^{(X)}_f(x,y) \defeq \psi^{(X)}(f(x), f(y))$.
It is possible to define $f$ by random projection such that $\embsize$ is constant in the document length $\maxtoks_y$, and with high probability $\psi^{(X)}_f$ is rank preserving with respect to $\Count_{0,1}$ for queries without repeating terms.

\begin{theorem}
Let $\maxtoks_X \geq 1$ be an upper bound on the number of tokens in a query. Let $x_t, y_t \in \indies_{\vocsize}$ be indicator vectors. Given $\beta > 0$, let $A \in \reals^{\embsize \times \vocsize}$ be a random projection such that $\embsize \geq k_0 = {24 (2 + \beta) \maxtoks_X^2 \ln \vocsize}.$ Then  with probability $\geq 1 - \vocsize^{-\beta}$, $\psi_f^{(X)}$ is rank preserving with respect to $\Count_{0,1}(x), \set{X}, \set{Y}$ for queries without repeated terms.
\end{theorem}
\begin{proof}
By the Johnson-Lindenstrauss lemma, for all $x, y$ in a set of size $\vocsize$,
\begin{equation}
\left| ||Ax - Ay||^2 - ||x - y||^2 \right| \leq  \epsilon ||x - y||^2,
\end{equation}
with probability $\geq 1 - \vocsize^{-\beta}$ if $A$ has dimension $\geq k_0 = {6 (2 + \beta) \epsilon^{-2} \ln \vocsize}$.
Because $||x||^2 = ||y||^2 = 1$ for all $x, y \in \indies_{\vocsize}$, by Lemma~\ref{lem:distances-and-products} this is equivalent to a bound on inner product errors, $    \left| \iprod{Ax_t}{Ay_{t'}} - \iprod{x_t}{y_{t'}} \right| \leq \epsilon.
$
Set $\epsilon := \frac{1}{2 \maxtoks_X}$. Because $\iprod{x_t}{y_{t'}} \in \{0, 1\}$, an error of $\epsilon = \frac{1}{2 \maxtoks_X} < \frac{1}{2}$ ensures  ${(\iprod{x_t}{y_{t'}} > \frac{1}{2})} \Rightarrow {(\iprod{f(x_t)}{f(y_{t'})} > \frac{1}{2})}.$ 
Thus, the attention scores $a_{x,y}(t,t')$ are identical after projection through $f$. Each $a_{x,y}(t,t')\iprod{f(x_t)}{f(y_{t'})}$ contributes an error ${< \frac{1}{2 \maxtoks_X z_{x,y}(t)}}$, and there are $z_{x,y}(t)$ such terms for each $t$. The total error for each query token is then ${< \frac{1}{2 \maxtoks_X}}$, and so ${|\psi^{(X)}_f(x,y) - \psi^{(X)}(x,y)| < \frac{1}{2}}$. By Lemma~\ref{lem:hard-attention-is-rank-preserving}, $\psi^{(X)}(x,y) = \iprod{\Count_{0,1}(x)}{\Count_{0,1}(y)}$ when $x$ has no repeating terms.  As argued in \autoref{thm:epsilon-precision-simple-inner-product}, errors ${<\frac{1}{2}}$ are rank preserving for simple inner product.
%Because simple inner product moves in unit %increments, errors ${< \frac{1}{2}}$ will not change any rankings.
\end{proof}
\commentout{
\begin{remark}
The dependence on $\maxtoks_X$ can be removed by applying a thresholding function to the inner product $\iprod{x_t}{\overline{y}_t}$, resulting in the score $\sum_{t=1}^{\maxtoks_x} 1[\iprod{x_t}{\overline{y}_t} > \frac{1}{2}].$ While beneficial in theory, this change defeat one of the main practical advantages of word embeddings, which is their ability to match near-synonyms in the query. Also, because queries are usually much shorter than documents, the dependence on $\maxtoks^2_X$ does not have a significant practical impact.
\end{remark}}

Attention enables the use of word encodings whose size is constant with respect to document length. This lends theoretical support to empirical findings that attention improves over dual encoder-style translation models on long inputs, such as for the translation of long sentences~\cite{bahdanau2014neural}.
While it is still necessary to store the integer identifiers of all terms in each document, the more practical impediment for the use of cross attention is the cost of computing $O(\maxtoks_x \maxtoks_y)$ inner products for each document-query pair.
%% I think the below statement would require more explanation if we were to include it. -J
%, without known algorithms for fast approximate search. 

%We explore this time-space tradeoff empirically in the next section.
%\kristina{I don't think we have explored the time-space tradeoff systematically.}
%\jacob{okay, maybe later :)}

Although this analysis has focused on the ability of cross attention to replicate simple inner product retrieval, we can also use contextualized embeddings in $x_t$ and $y_t$ to pool information across tokens and gain additional linguistic sensitivity. This is outside the scope of our theoretical analysis and must be evaluated empirically.



==> analyzing_dual_encoders.tex <==
\vspace{-.1cm}
\section{Analyzing Dual Encoder Retrieval}
%\vspace{-.1cm}

A query or a document is a sequence of words drawn from some vocabulary $\set{V} = \{1, 2, \ldots \vocsize\}$.\footnote{We represent each word  as an integer for convenience.} %\footnote{See \autoref{tab:notation} in the appendix for a summary of mathematical notation.}
Throughout this section we assume a representation of queries and documents typically used in sparse bag-of-words models; each query $q$ is a vector in $\reals^\vocsize$ where $\vocsize$ is the vocabulary size, and similarly each document $d$ is a vector in $\reals^\vocsize$. We take the inner product $\langle q, d \rangle$ to be the relevance score of document $d$ for query $q$. For part of this section, we will focus on the simple case of boolean inner product, where
$q$ and $d$ are elements of $\{0,1\}^{\vocsize}$, with $d_i=1$ appears at least once in the document, and $q_i$ defined analogously. Extensions to \tfidf~\cite{sparck1972statistical} and \bm~\cite{robertson2009probabilistic} are discussed in Section~\ref{sec:nonboolean}.
%: documents are ranked by their relevance scores for a given query.

\commentout{Throughout this section we assume a restricted bag-of-words representation of queries and documents, where a query $q$ is a vector in $\reals^\vocsize$ where $\vocsize$ is the vocabulary size, and similarly a document $d$ is also a vector in $\reals^\vocsize$. We take the inner product $\langle q, d \rangle$ to be the relevance score of document $d$ for query $q$: documents are ranked by their relevance scores for a given query.} 
%Common examples of encodings of queries and documents in $\reals^{\vocsize}$ are:
\commentout{We will compare compressive dual encoder retrieval against classical bag-of-words retrieval models, which can be viewed as encoding each document as its bag-of-words vector, possibly after scaling. We will write the bags-of-words for the query and document as $q,d  \in \mathbb{N}^{\vocsize},$ using $q$ and $d$ to refer to these word counts in this section of the paper. The relevance score for document $d$ against query $q$ is written as
$\psi(q,d) \defeq \iprod{q}{d}$}
%This generalizes the following special cases:}
%\begin{itemize}
%\item Simple inner product retrieval, where $q$ and $d$ are in the space $\{0,1\}^{\vocsize}$, with $d_i$ and $q_i = 1$ iff word $i$ appears at least once in the sequence. 
%The query vector $q$ is defined analogously.
%\item {\small {TF-IDF}}~\cite{sparck1972statistical}, where $d_i = 0$ if word $i$ does not appear in the document, and the word   $\text{count}(i)$ times the square root of its inverse document frequency otherwise, and \bm~\cite{robertson2009probabilistic}, which additionally uses a  function $\tau(\text{count}(i))$  that  ``squashes'' this count to a fixed range.
%\end{itemize}

%As shown in \autoref{fig:1-retrieve-passage-contain-q}, \bm offers strong performance in comparison with a \bert-based dual encoder.
%These encodings can also be applied to bigram counts, with an increase of dimensionality to $\vocsize^2$.

We will compare relevance scores $\iprod{q}{d}$ with compressive dual encoders, for which we write $f(d)$ and $f(q)$ to indicate compression of $d$ and $q$ to $\reals^{\embsize}$, with $\embsize < \vocsize,$ and where $\embsize$ does not vary with the document length. We write the relevance score as the inner product $\iprod{f(q)}{f(d)}$. (In \autoref{sec:attention}, we consider encoder functions that apply to sequences of tokens rather than vectors of word counts.)


A fundamental question is how the capacity of dual encoder retrieval varies with the embedding size $\embsize$. A tractable proxy for capacity is \term{fidelity}: how much can we compress the input while maintaining the ability to mimic the performance of bag-of-words retrieval?
To answer this question, we will relate the embedding size to bounds on the absolute difference between inner products $|\iprod{f(q)}{f(d)} - \iprod{q}{d}|$. 

%\subsection{Tail bounds and ranking accuracy}
%\label{sec:tail-bounds-and-accuracy}
%Suppose that the inner product deviation is bounded,
%\begin{equation}
%|\psi_f(q,d) - \psi(q,d)| < \alpha.
%\end{equation}


\begin{definition}
\label{def:rank-preservation}
Let $\set{Q} \subseteq \reals^{\vocsize}$ be a set of queries and let $\set{D} \subseteq \reals^{\vocsize}$ be a set of documents. An encoder $f : \reals^{\vocsize} \to \reals^{\embsize}$ is \term{rank preserving} over $\set{D}$ and $\set{Q}$ iff
%\kristina{Should this be if and only if instead?; mike - changing this to iff} 
for all triples $(q, d_1, d_2) \in \set{Q} \times \set{D} \times \set{D}$, pairwise relevance rankings are preserved after encoding:\footnote{The encoder is free to break ties arbitrarily.}
\commentout{: if $\iprod{q}{d_1} = \iprod{q}{d_2}$ then any relationship between $\iprod{f(q)}{f(d_1)}$ and $\iprod{f(q)}{f(d_2)}$ is permitted.}
\vspace{-2ex}
\begin{equation}
\begin{split}
    & (\iprod{q}{d_1} > \iprod{q}{d_2}) \\
    & \Rightarrow (\iprod{f(q)}{f(d_1)} > \iprod{f(q)}{f(d_2)}).
\end{split}
\end{equation}
\end{definition}

We wish to guarantee that a compressive encoder is rank preserving if it is sufficiently precise. 
Much of the literature on dimensionality reduction~\cite[e.g.,][]{vempala2004random} characterizes precision in terms of distances:
\begin{definition}
Encoder $f : \reals^{\vocsize} \to \reals^{\embsize}$ is \term{$\epsilon$-precise} for query $q \in  \reals^{\vocsize}$ and document $d \in \reals^{\vocsize}$ iff,
%if for all $q, d \in \reals^{\vocsize}$,
\begin{equation}
\left| ||f(q) - f(d)||^2 - ||q - d||^2 \right| \leq \epsilon ||q-d||^2.
%    \Pr \left\{ \left| ||f(x) - f(y)||^2 - ||x - y||^2 \right| \leq (1 + \epsilon) ||x-y||^2 \right\} \geq 1-\rho
\end{equation}
We say $f$ is $\epsilon$-precise over \emph{sets} $\set{Q}$ and $\set{D}$ when $f$ is $\epsilon$-precise over all $(q,d) \in \set{Q} \times \set{D}$.
\end{definition}

\begin{comment}
% incorporated -J
Suggested revision from Mike:

\newcommand{\qtext}{\mathcal{Q}'}

Assume a set of queries $\qtext$

\begin{definition}
An encoder $f : \reals^{\vocsize} \to \reals^{\embsize}$ is \term{$\epsilon$-precise} over $(\mathcal{Q}, \mathcal{D})$ if for all $(q, d) \in \mathcal{Q} \times \mathcal{D}$,
\begin{equation}
\left| ||f(q) - f(d)||^2 - ||q - d||^2 \right| \leq (1 + \epsilon) ||q-d||^2,
%    \Pr \left\{ \left| ||f(x) - f(y)||^2 - ||x - y||^2 \right| \leq (1 + \epsilon) ||x-y||^2 \right\} \geq 1-\rho
\end{equation}
\end{definition}
\end{comment}

The precision of distances can be related to inner products by the following lemma, adapted from \newcite[][corollary 19]{ben2002limitations}.

\begin{lemma}
\label{lem:distances-and-products}
Assume an encoder $f : \reals^{\vocsize} \to \reals^{\embsize}$ is \term{$\epsilon$-precise} for  $q \in \reals^{\vocsize}$ and  $d \in \reals^{\vocsize}$. It follows that
\begin{align}
    \left| \iprod{f(q)}{f(d)} - \iprod{q}{d} \right| \leq & \frac{\epsilon}{2} (||q||^2 + ||d||^2).
\label{eq:dists-to-products-in-paper}
\end{align}
\end{lemma}

%\begin{proof}
%See \cite{ttipaper}.
%See \autoref{app:proof-of-distances-and-products}.
%\end{proof}



% We will focus on the case of scaled inner product retrieval, in which $||g(q)|| = ||g(d)|| = 1$. 
% In this case, for an $\epsilon$-precise encoder, the inner product error is bounded by $\pm \epsilon$.
We now state a theorem that links rank preservation and $\epsilon$-precision in the case where each query or document is a vector in $\{0, 1\}^{\vocsize}$:

\begin{theorem}
Let $\set{Q} \subseteq \{0, 1\}^{\vocsize}$ be a set of queries and let $\set{D} \subseteq \{0, 1\}^{\vocsize}$ be a set of documents. Assume constants $\maxterms_q$ and $\maxterms_d$ such that $\forall q \in \set{Q}$, $\sum_{i=1}^v |q_i| < \maxterms_q$ and $\forall d \in \set{D}$, $\sum_{i=1}^v |d_i| < \maxterms_d$.
If encoder $f$ is $\epsilon$-precise for $\set{D}, \set{Q}$ with $\epsilon \leq (\maxterms_q + \maxterms_d)^{-1}$, 
then it is rank preserving over $\set{D}$ and $\set{Q}$.
%with probability $1-\rho$, then it is rank-preserving with probability $1 - |\mathcal{D}|^2 |\mathcal{Q}| \rho$ with respect to simple inner product retrieval.
\label{thm:epsilon-precision-simple-inner-product}
\end{theorem}
\begin{proof}
Under the assumption that each query or document is a vector in $\{0, 1\}^{\vocsize}$, if $\iprod{q}{d_1} > \iprod{q}{d_2}$ then the minimum possible margin is $\iprod{q}{d_1} - \iprod{q}{d_2} = 1$. Thus, if $f$'s errors for each document-query inner product are $ < \frac{1}{2}$, then $f$ is rank preserving. 
If $\sum_{i=1}^{\vocsize} |d_i| < \maxterms_d$ then $||d|| < \sqrt{\maxterms_d}$, and analogously, $||q|| < \sqrt{\maxterms_q}$. Let $\epsilon = (\maxterms_q + \maxterms_d)^{-1}$ and plug this value into \autoref{eq:dists-to-products-in-paper}:
\begin{align}
    \frac{\epsilon}{2}(||q||^2 + ||d||^2)
    = \frac{1}{2}\frac{||q||^2 + ||d||^2}{\maxterms_q + \maxterms_d}
    < \frac{1}{2},
\end{align}
because $\maxterms_q > ||q||^2$ and $\maxterms_d > ||d||^2$ for all $d, q$.
\end{proof}

\commentout{
\paragraph{\tfidf and \bm.}
%In principle a similar analysis can be applied to more complex bag-of-words models. 
%For scaled inner product retrieval, the minimum margin arises when $\iprod{q}{d_1} = \iprod{q}{d_2}$ but $||d_1|| < ||d_2|| = \maxnorm_d$, so that rank preservation requires a precision of $\epsilon \leq \frac{1}{2}(\maxnorm_q \maxnorm_d^2)^{-1}.$ 
\newtext{Both \tfidf~\cite{sparck1972statistical} and \bm~\cite{robertson2009probabilistic} can be written as inner products between bag-of-words representations of the document and query as described earlier in this section.
Set the query representation $\tilde{q}_i = q_i \times \textsc{idf}_i$, where $q_i$ indicates the presence of the term in the query and $\textsc{idf}_i$ indicates the inverse document frequency of term $i$. The TF-IDF score is then $\iprod{\tilde{q}}{d}$. For BM25, we must define a vector $\tilde{d} \in \reals^{\vocsize}$, with each $\tilde{d}_i$ a function of the count $d_i$ and the document length, along with several hyperparameters~\cite{robertson2009probabilistic}. The key point is that for every document $d$ there exists some $\tilde{d} \in \reals^{\vocsize}$ such that ${\iprod{\tilde{q}}{\tilde{d}} = \text{\bm}(q,d)}$. %Furthermore, for documents of average length, $\tilde{d}_i \in [1, k_1 + 1]$, with $k_1 \in [1.2, 2]$
}

\newtext{Unfortunately, it is difficult to theoretically analyze this inner product. First, the norm $||\tilde{d}||$ has a complex relationship with document length, which appears in the denominator of the \bm relevance function. Second, while in boolean dot product it is possible to eliminate ranking errors by bounding dot product errors by $\frac{1}{2}$, it is more difficult to derive the minimum ranking margin in \bm and \tfidf. Indeed, this margin depends in part on the query length: because each term may have a unique inverse document frequency, the minimum margin $\min_{d_1, d_2} \iprod{\tilde{q}}{d_1} - \iprod{\tilde{q}}{d_2}$ can decrease with the number of terms in the query, as each additional term creates more ways in which two documents can receive nearly the same score. This necessitates a more precise encoding of $\tilde{q}_i$ and $\tilde{d}_i$, which in turn necessitates higher encoding dimension. We therefore leave the theoretical analysis of these more elaborate ranking functions to future work. See \autoref{fig:bm25-dp-approx} for an empirical analysis of the relationship of dual encoding and \bm for random projections. Our experiments in \autoref{sec:experiments} also focus on \bm due to its strong performance on classical information retrieval benchmarks.}

% Nonetheless, given a constraint on query and document lengths, it is theoretically possible to establish \emph{some} minimum margin, so there must exist an $\epsilon$ which guarantees that an encoder is rank-preserving, and which can be related to the document and query length.
}

==> experimental-results-table-desc.tex <==
The MSMARCO passage ranking task focuses on ranking passages, where it contains 1,010,916 queries on a collection of 8,841,823 passages. The document ranking task is based on source documents, which contains passages in the passage ranking task. The full corpus is 3,213,835 documents and the training set has 367,013 queries. The training set contains approximately 532k queries. The development set contains 6,980 queries. For TRECCAR dataset, the input query is the concatenation of a Wikipedia article title with the title of one of its section. We follow the setup of \newcite{passage-rerank} and use automatic annotations, where the training set has 2323949 queries, 583014 queries for dev and 2254 queries for test set. \yi{Also talk about average length of each dataset?}

==> general_limits.tex <==
\section{General Limits on Dual Encoders}
\label{sec:limitations}
\commentout{
Given the pessimistic results on embedding size for random projections, it is natural to ask whether more compact representations could be obtained from more expressive encoding functions, such as transformer networks~\cite{vaswani2017attention}. In general, the answer is no.}

The previous sections introduced upper bounds on the required embedding dimension. An important question is whether there are matching lower bounds. We do not have a full answer to this question, but the following theorem states a lower bound that may be relevant:

\begin{theorem}[\newcite{larsen2017optimality}]
\label{thm:larsen-nelson}
%\newcite{larsen2017optimality} consider
For any $\vocsize, \numdocs \geq 2$ and %$\epsilon \in ( \log^{.5001} \numdocs / \sqrt{ \min  \{ \numdocs, \vocsize \}}, 1)$\footnote{When $\epsilon < (\min\{\numdocs, \vocsize\})^{-1/2}$, the term $\epsilon^{-2} > \min \{ \numdocs, \vocsize \}$. But it is always possible to construct a representation of size $\min \{\numdocs, \vocsize\}$, either by using $X$ directly (when $\vocsize \leq \numdocs$) or by projecting onto the span of $X$.
%The theorem does not address the range $\epsilon \in ((\min\{\numdocs, \vocsize\})^{-1/2}, (\ln \numdocs / (\min\{\numdocs, \vocsize\}))^{1/2}]$.
%}
for precision $\epsilon$\footnote{The theorem applies to ${\epsilon \in ( \log^{.5001} \numdocs / \sqrt{ \min  \{ \numdocs, \vocsize \}}, 1)}$. Values outside this range are unlikely to be relevant in practice.}
there exists a set of points $X \subset \reals^{\vocsize}$ such that any map 
$f : X \to \reals^{\embsize}$ that is $\epsilon$-precise must have $\embsize = \Omega(\epsilon^{-2} \ln \numdocs).$
\end{theorem}
%% shortened but included the actual range for accuracy -J
%\kristina{Can we omit all of the discussion of the range of $\epsilon$ this applies to and just say the range of practical interest; this will also save a footnote.}
%\jacob{i'm open to it but "range of practical interest" is a little informal for a theorem. how would you put it? } \kristina{I would just say precision $\epsilon$ in the theorem and add a footnote saying for brevity here we omit restrictions on the range of $\epsilon$ which do not impact the case of practical interest.}
\autoref{thm:larsen-nelson} states that no encoder $f$ will be $\epsilon$-precise for all vector sets unless $\embsize$ grows with $\epsilon^{-2}$.\footnote{\newtext{A related bound can be derived specifically for additive errors on inner products: for sets of vectors whose norms are $\leq 1$, any representation that preserves inner products to an additive error bounded by $\epsilon$ must require a number of bits that grows asymptotically with $\epsilon^{-2}$~\cite{alon2017optimal}.}}
\commentout{Thus, low-dimensional compressive encodings of large documents are unlikely to accurately replicate inner products on bags-of-words, regardless of how the encoder is computed.}
However, this requires the assumption that the documents of interest are ``hard to embed'' in the sense of \citeauthor{larsen2017optimality}.
Their proof constructs a set of sets $\mathcal{X} = \{X_1, X_2, \ldots \}$, where each $X_i$ is composed of $k$-sparse vectors, similar to bags-of-words. 
%% how about this? -J
%\kristina{I think we can omit the above three sentences starting from ``Their proof ..''.}
%\jacob{The point is to show that the construction is not too exotic from an NLP perspective. I think Ming-wei asked about this on Friday.}
%\kristina{Maybe it could be made shorter, saying that the proof uses a set of sets of $k$-sparse vectors, similar to bag-of-words, and shows that the overwhelming majority of them cannot be embedded precisely in lower-dimensional space. }
However, the theorem does not imply that \emph{every} such set of vectors is hard to embed precisely.
Consider a simple generative model in which all documents are generated deterministically from a few topics: this particular $X$ could be encoded compactly by indexing which topic is responsible for each document.
Are real document collections more like this, or more like the ``hard" vector sets constructed by \citeauthor{larsen2017optimality}?

There are further questions about the applicability of this theorem to real texts. We have focused on ensuring the inner products are sufficiently precise so as to preserve \emph{every} pairwise ranking. It is possible that the overwhelming majority of rankings could be preserved with lower-precision inner products; see, e.g., work on approximate nearest neighbors~\cite{indyk1998approximate}.  Finally, in practice the dual encoder model trades fidelity for the ability to generalize across related words and phrases, and this may be a worthwhile tradeoff in real tasks of interest. Lacking theoretical tools to settle these questions, we present a set of empirical investigations in \autoref{sec:experiments}. But first we relate this theoretical framework to attentional architectures, which abandon the inner product retrieval model in favor of more fine-grained treatment of the relationship between queries and documents.

%Until this theoretical gap is filled, the applicability of this analysis depends in part on empirical results, as described in the following sections.

%% need to think about this some more, probably not for this paper
%\subsection{Extensions}
%Suppose you have a function $g: X \to \reals$ that is smooth in the sense that $(g(x_1) - g(x_2))^2 \leq C ||x_1 - x_2||^2$ for some $C > 0$. Depending on the value of $C$, an embedding function that does not preserve distances would be able to 




==> projections.tex <==
\section{Dual Encoder Retrieval by Projection}
\label{sec:projections}
To establish baselines on the performance of compressive dual encoder retrieval, we now consider encoders based on \term{random projections}~\cite{vempala2004random}.
%which we call \derp (dual encoder retrieval by projection). 
The encoder is defined as $f(x) = Ax,$ where $A \in \reals^{k \times v}$ is a random matrix.
%% Cut for space -J
%We consider two types of distributions over $A$: Rademacher embeddings and isotropic Gaussians.
%Both encoders can achieve $\epsilon$-precision with probability $1 - \rho$ if the embedding size is $\Omega(\epsilon^{-2} \ln \rho^{-1})$.
%%\jacob{If we're still in trouble for space, we can save 1/4 page by combining the Rademacher and Gaussian embeddings.}
%% Mike: just doing this now
In \term{Rademacher embeddings}, each element $a_{i,j}$ of the  matrix $A$ is sampled with equal probability from two possible values: $\{-\frac{1}{\sqrt{\embsize}},\frac{1}{\sqrt{\embsize}}\}$.
In \term{Gaussian embeddings}, each $a_{i,j} \sim N(0,\embsize^{-1/2})$. 
%That is, each element of the projection matrix is normally distributed with zero mean and variance $\embsize^{-1}$. 
The following theorem applies:

\commentout{
In both cases, it is possible to precisely characterize the inner products of word embeddings, which are the columns of $A$.
From this, it is possible to derive a bound on the error ${|\iprod{f(q)}{f(d)}-\iprod{q}{d}|}$ with high probability.}

\begin{theorem}[\newcite{achlioptas2003database}]
Given a set of queries $\set{Q} \subseteq \reals^v$ and documents $\set{D} \subseteq \reals^v$ define $\numdocs = |\set{Q} \cup \set{D}|$. Given $\epsilon, \beta > 0$ let
$
k_0 = \frac{4 + 2\beta}{\epsilon^2/2 - \epsilon^3/3} \ln \numdocs
$.
For integer $k \geq k_0$ let $A$ be a $k \times v$ dimensional matrix of Rademacher or Gaussian embeddings and let $f(x) = Ax$. Then with probability at least $1 - \numdocs^{-\beta}$, $f$ is $\epsilon$-precise over all $(q, d) \in \set{Q} \times \set{D}$.
\label{thm:dasgupta-JL}
\end{theorem}


\commentout{
\begin{theorem}[\newcite{achlioptas2003database}]
Let $f(x) = Ax$, with $A$ distributed as Rademacher embeddings, and 
let $\numdocs = |\set{Q} \cup \set{D}|$
Then $f$ is $\epsilon$-precise over all $(q, d) \in \set{Q} \times \set{D}$ with probability 
$\rho \geq 1 - \numdocs^{-\beta}$ if the embedding size is an integer satisfying 
$\embsize \geq \frac{4 + 2\beta}{\epsilon^2/2 - \epsilon^3/3} \ln \numdocs$.
\end{theorem}}

%\mike{changed this from $\epsilon^2/2 - \epsilon^3/3 \leq  \epsilon^2/3$ I think this was an error? Also thought it would be good to be concrete about $c$?}
%% you are right -J
\begin{remark}
When $\epsilon \leq \frac{1}{2}$, we can use $\epsilon^2/3 \leq {\epsilon^2/2 - \epsilon^3/3}$ to obtain a simpler but looser bound ${\embsize \geq 6 (2 + \beta) \epsilon^{-2} \ln \numdocs}$. 
%In comparison with \autoref{thm:hoeffding-rademacher}, this bound avoids the terms $\ln ||q||_0 + \ln ||d||_0$ but has a worse constant factor.
\end{remark}

\commentout{
\subsection{Gaussian embeddings}
In practice word embeddings are typically dense vectors. We now consider a random projection matrix $A = [a_{i,j}] \in \reals^{\embsize \times \vocsize}$, with each $a_{i,j} \sim N(0,\embsize^{-1/2})$. That is, each element of the projection matrix is normally distributed with zero mean and variance $\embsize^{-1}$, and each column is a word embedding of dimension $\embsize$. To characterize this model, we restate a theorem from \newcite{dasgupta2003elementary}, which is a sharper version of the classical lemma of \newcite{johnson1984extensions}:
\begin{theorem}[\newcite{dasgupta2003elementary}; see also \newcite{achlioptas2003database}]
Given a set of queries $\set{Q} \subseteq \reals^v$ and documents $\set{D} \subseteq \reals^v$ define $\numdocs = |\set{Q} \cup \set{D}|$. Given $\epsilon, \beta > 0$ let
\[
k_0 = \frac{4 + 2\beta}{\epsilon^2/2 - \epsilon^3/3} \ln \numdocs
\]
For integer $k \geq k_0$ let $A$ be a $k \times v$ dimensional matrix with each $a_{i,j} \sim N(0,\embsize^{-1/2})$ and let $f(x) = Ax$. Then with probability at least $1 - \numdocs^{-\beta}$, $f$ is $\epsilon$-precise over all $(q, d) \in \set{Q} \times \set{D}$.
\end{theorem}

\commentout{
\begin{theorem}[\newcite{dasgupta2003elementary}; see also \newcite{achlioptas2003database}]
Let $f(x) = Ax$, with $A$ distributed as $a_{i,j} \sim N(0,\embsize^{-1/2})$. 
Let $\numdocs = |\set{Q} \cup \set{D}|$.
Then $f$ is $\epsilon$-precise over all $(q, d) \in \set{Q} \times \set{D}$ with probability 
$\rho \geq 1 - \numdocs^{-\beta}$ if the embedding size is an integer satisfying 
$\embsize \geq \frac{4 + 2 \beta}{\epsilon^2/2 - \epsilon^3/3} \ln \numdocs$.
\end{theorem}}
 
\begin{remark}
This bound is the same as the one obtained by \newcite{achlioptas2003database} for Rademacher embeddings. Again, when $\epsilon \leq \frac{1}{2}$, we can obtain a simpler but looser bound in terms of $\epsilon^{-2}$.
\end{remark}}

\commentout{
Both Rademacher and Gaussian random projections are $\epsilon$-precise when the embedding size grows with $\epsilon^{-2}$, the squared inverse error.\footnote{The same asymptotic dependence arises from the approximation of inner products by random hashing functions~\cite{weinberger2009feature}.}
}

%\autoref{thm:epsilon-precision-simple-inner-product} states that a compressive encoder is rank preserving if $\epsilon \leq \frac{1}{\maxterms_q + \maxterms_d}$.
\autoref{thm:epsilon-precision-simple-inner-product} states that  if a compressive encoder is $\epsilon$-precise with  $\epsilon \leq \frac{1}{\maxterms_q + \maxterms_d}$, then it is rank preserving relative to boolean dot product retrieval. Combining this with \autoref{thm:dasgupta-JL} and substituting $\numdocs = |\set{Q} \cup \set{D}| \leq |\set{Q}| + |\set{D}|$, if a random projection has size
\begin{equation}
    \embsize \geq 6(2 + \beta) (\maxterms_q + \maxterms_d)^2 \ln (|\set{Q}| + |\set{D}|),
\end{equation} it is rank preserving relative to boolean retrieval with probability at least $1 - \numdocs^{-\beta}$. 


%Combining this with \autoref{thm:dasgupta-JL} and substituting $\numdocs = |\set{Q} \cup \set{D}| \leq |\set{Q}| + |\set{D}|$, random projections are rank preserving with probability $1 - \numdocs^{-\beta}$ when
%\begin{equation}
%    \embsize \geq 6(2 + \beta) (\maxterms_q + \maxterms_d)^2 \ln (|\set{Q}| + |\set{D}|).
%\end{equation}

\newtext{The bound requires} that the size of the embeddings  grow with the square of the number of unique terms in the query and document.\footnote{In natural language, the number of unique terms usually grows sublinearly with the number of tokens $\maxtoks$. A classical model is $\maxterms \propto \maxtoks^\beta$, with $\beta < 1$~\cite{herdan1960type,heaps1978information}. %See \newcite{gerz-etal-2018-language} for a recent empirical cross-lingual comparison.
}\newtext{Although this is an upper bound and may be too pessimistic, empirical studies and related theoretical work may support a similar asymptotic growth of a lower bound (see ~\autoref{sec:nonboolean} and ~\autoref{sec:lowerbound}).}
%\newtext{\autoref{thm:dasgupta-JL} is tight in the sense that there exist vector sets that cannot be embedded to precision $\epsilon$ unless the dimensionality of the embedding grows with $\epsilon^{-2}$, even when arbitrary (e.g. non-linear) projections are used (see \autoref{sec:limitations}).


%\newtext{
\subsection{Rank preservation for more general sparse models}
\label{sec:nonboolean}
We now introduce results for more general sparse models such as  \tfidf~\cite{sparck1972statistical} and \bm~\cite{robertson2009probabilistic}, which employ more powerful weighting schemes than boolean representations.
Both \tfidf and \bm can be written as inner products between bag-of-words representations of the document and query.
Set the query representation $\tilde{q}_i = q_i \times \textsc{idf}_i$, where $q_i$ indicates the presence of the term in the query and $\textsc{idf}_i$ indicates the inverse document frequency of term $i$. The TF-IDF score is then $\iprod{\tilde{q}}{d}$. For BM25, we must define a vector $\tilde{d} \in \reals^{\vocsize}$, with each $\tilde{d}_i$ a function of the count $d_i$ and the document length, along with several hyperparameters~\cite{robertson2009probabilistic}. The key point is that for every document $d$ there exists some $\tilde{d} \in \reals^{\vocsize}$ such that ${\iprod{\tilde{q}}{\tilde{d}} = \text{\bm}(q,d)}$. %Furthermore, for documents of average length, $\tilde{d}_i \in [1, k_1 + 1]$, with $k_1 \in [1.2, 2]$


For \bm and other classical retrieval models, the minimum non-zero margin $\iprod{q}{d_1} - \iprod{q}{d_2}$  can be much smaller than $1$ and is dataset dependent. For example, the minimum observed margin for \bm for the MS MARCO documents dataset (see ~\autoref{sec:ir-eval}) is less than $ 10^{-5}$. Although such close rankings are difficult to preserve with random projections, the majority of rankings for triples $(q,d_1,d_2)$ we care about may be easier to preserve.

Here we derive a lower bound on the probability that a random projection will preserve a specific pairwise ranking of interest, depending on the dimensionality $k$ and properties of the vectors $q$, $d_1$, and $d_2$. Without loss of generality, we assume that the sparse model prefers $d_1$, meaning that $\iprod{q}{d_1} > \iprod{q}{d_2}$. An application of the Johnson-Lindenstrauss lemma gives the following bound on the error probability for any triple $(q, d_1, d_2)$:

\commentout{
For convenience, define
\[
\delta(q, d_1, d_2) = \frac{q \cdot (d_1 - d_2)}{||q|| ||d_1 - d_2||}
\]

We term $\delta$ the \emph{normalized margin} for the triple $q, d_1, d_2$.
}

\newcommand{\nmarg}[1]{\ensuremath \delta\left(#1\right)}
\begin{lemma}
Define a matrix $A \in \reals^{k \times d}$ consisting of random Rademacher or Gaussian embeddings.  For any $(q, d_1, d_2)$ triple, define the \term{normalized margin} $\nmarg{q, d_1, d_2} = \frac{\iprod{q}{d_1 - d_2}}{||q|| \times ||d_1 - d_2||}$. Define $\bar{q} = A q$,
$\bar{d}_1 = A d_1$, and $\bar{d}_2 = A d_2$. Assume $\delta(q, d_1, d_2) > 0$. Then
\begin{equation}
    \Pr(\bar{q} \cdot (\bar{d}_1 - \bar{d}_2) \leq 0) \leq g(\nmarg{q, d_1, d_2}, k),
\end{equation}
where $g(\epsilon, k) = 4 \exp {( - k(\epsilon^2 - \epsilon^3)/4)}$
\end{lemma}

\begin{proof} 
Define $\tilde{q} = q/||q||$ and $\tilde{d}_{1,2} = (d_1 - d_2)/||d_1 - d_2||$. Note that 
\[
\delta(q, d_1, d_2) = \tilde{q} \cdot \tilde{d}_{1,2}
\]

From corollary 2.1 of \url{https://ttic.uchicago.edu/~gregory/courses/LargeScaleLearning/lectures/jl.pdf}, for any $\delta$ we have
\[
\Pr( | \tilde{q} \cdot \tilde{d}_{1,2} - (A \tilde{q}) \cdot (A \tilde{d}_{1,2})| \geq \delta)
\leq
4 \exp { (- k(\delta^2 - \delta^3)/4)}
\]
This in turn implies
\[
\Pr(  (A \tilde{q}) \cdot (A \tilde{d}_{1,2}) \leq \tilde{q} \cdot \tilde{d}_{1,2} - \delta)
\leq
4 \exp { (- k(\delta^2 - \delta^3)/4)}
\]
%(actually we only used 1 side of the JL bound here, so perhaps we can reduce the RHS by a factor of 2).

Under the assumption that $\tilde{q} \cdot \tilde{d}_{1,2} = \delta(q_1, d_1, d_2) > 0$ we have
\[
\Pr(  (A \tilde{q}) \cdot (A \tilde{d}_{1,2}) \leq 0)
\leq 4 \exp {( - k(\delta^2 - \delta^3)/4)}
\]
where $\delta = \delta(q_1, d_1, d_2)$, which in turn implies
\[
\Pr(  (A {q}) \cdot (A {d}_{1,2}) \leq 0)
\leq 4 \exp {( - k(\delta^2 - \delta^3)/4)}
\]
where $\delta = \delta(q_1, d_1, d_2)$, proving the lemma. \end{proof}

For a given $(q,d_1,d_2)$ example, this bound gives as a way to select an embedding dimension $k$ such that it can be ranked correctly with high probability. For example, to achieve probability of error less than $\gamma$, we can select $k$ such that:
$4 \exp { - k(\delta^2 - \delta^3)/4} < \gamma$, or equivalently:
$k > \frac{1}{\delta^2-\delta^3}4(\log \frac{4}{\gamma})$.

Note that for a fixed query $q$ and margin $\iprod{q}{d_1}-\iprod{q}{d_2}$, $\delta$ becomes smaller as  $||d_1 - d_2||$ grows. For both boolean and \bm dot product retrieval, the maximum $||d_1 - d_2||$ increases with the number of unique tokens in the documents.

To see whether the predicted relationship between $\delta$ and the minimum dimensionality $k$ of a random projection that can preserve the pair-wise ranking for a triple $(q,d_1,d_2)$ with normalized margin $\delta$ may provide a too pessimistic picture, we measure this relationship on a real natural language text retrieval problem. 

Using the MS MARCO document retrieval dataset (see ~\autoref{sec:ir-eval}) for data processing details, we evaluate the ability of Rademacher random projections to achieve accuracy of at least $95\%$ on pairwise rankings $(q,d_1,d_2)$, with respect to both boolean (Figure \ref{fig:simple-dp-approx-rankings}) and \bm sparse representations (Figure \ref{fig:bm25-dp-approx-rankings}).

Input triples $(q,d_1,d_2)$ are binned by their corresponding $\frac{1}{\delta^2-\delta^3}$ and represented on the $x$ axes. The $y$ axes show the minimum dimension projection $k$ that reached pairwise ranking error of less than $.05$ for the corresponding bin. We tested a grid of $50$ values of $k$ (examples that could not be ranked with the desired accuracy given the explored range were excluded.) The empirical lower bound obtained from these experiments displays a linear relationship with  $\frac{1}{\delta^2-\delta^3}$, matching the theoretical upper bound (ignoring constants).
%}
\commentout{To relate the embedding precision to the inner product error and ranking performance, we perform empirical evaluations. In \autoref{fig:simple-dp-approx}, we examine naturally occurring documents from the inverse cloze task described in \autoref{sec:ict-unmasked}. 
We consider 200 candidate documents for each query, and compute the simple inner product of the boolean bag-of-bigram vectors ($\vocsize \approx 4.6\times 10^7$). 
We then group by $(\ell_q + \ell_d)^2$, and plot the minimum $\embsize$ such that the inner product of Rademacher projections achieves an average error ${< \frac{1}{2}}.$
\newtext{In \autoref{fig:bm25-dp-approx}, we use synthetic documents and queries to assess the fidelity of random projection with respect to \bm. Treating the \bm retrieval result as the gold standard, we plot the minimum $\embsize$ such that an inner product after Gaussian projection achieves a recall-at-one of at least $0.5$. Note that in this case we don't require approximation of all \bm dot products, but only assess how often the top \bm document is also ranked top by the projected representation.  Both figures show a linear relationship between the quantity $(\ell_q + \ell_d)^2$ and the minimum embedding size, as predicted by the theory.}}


\begin{figure}
    \centering
    %\framebox(200,100){}
    \includegraphics[width=.9\columnwidth]{figures/ind_delta.pdf}
    
    \caption{\small Min. $\embsize$ for Rademacher embeddings to approximate simple dot product pairwise rankings with average error ${<.05}$.
    %, for query-document pairs grouped by $(l_q + l_d)^2$.
    }
    \label{fig:simple-dp-approx-rankings}
\end{figure}

\begin{figure}
    \centering
    %\framebox(200,100){}
    % \includegraphics[width=.9\columnwidth]{figures/K_versus_BM25_squared_norm_doc_and_query.png}
    \includegraphics[width=.9\columnwidth]{figures/bm25_delta.pdf}
    \caption{\small Min. $\embsize$ for Rademacher embeddings to approximate \bm pairwise rankings with average error ${<.05}$.}
    \label{fig:bm25-dp-approx-rankings}
\end{figure}

\commentout{
\begin{figure}
    \centering
    %\framebox(200,100){}
    \includegraphics[width=.9\columnwidth]{figures/min_k_by_norm.pdf}
    
    \caption{\small Min. $\embsize$ for Rademacher embeddings to approximate simple dot product with average error ${<\frac{1}{2}}$.
    %, for query-document pairs grouped by $(l_q + l_d)^2$.
    }
    \label{fig:simple-dp-approx}
\end{figure}

\begin{figure}
    \centering
    %\framebox(200,100){}
    % \includegraphics[width=.9\columnwidth]{figures/K_versus_BM25_squared_norm_doc_and_query.png}
    \includegraphics[width=.9\columnwidth]{figures/K_versus_BM25.pdf}
    \caption{\small Min. $\embsize$ for Gaussian embeddings to approximate \bm with recall@1 $\geq 0.5$ \jacob{todo: use Rademacher embeddings to be consistent with fig 2}}
    \label{fig:bm25-dp-approx}
\end{figure}

}

%We now ask whether learned encoders might offer better results.

\subsection{Deriving Lower Bounds}
\label{sec:lowerbound}
This section has presented upper bounds on the dimensionality required for effective retrieval. An open question is whether related lower bounds can be derived, and under which assumptions such lower bounds hold. The work of \newcite{larsen2017optimality} which derives lower bounds on embedding size for arbitrary (linear or non-linear) embeddings is highly relevant to this question. \newcite{alongKlartag2017} derive related results for inner products.

==> recall_at_r_empirical.tex <==
\commentout{
\paragraph{Recall-at-$r$.} Next, we consider the ranking performance as measured in recall-at-$r$. For each query, we compute the normalized margin $\nmarg(q, d_1, d_r)$, where $d_1$ is the document that maximizes \bm for $q$, and $d_r$ is the document with the $r$th-smallest normalized margin. We then bin the queries by these margins, excluding bins for which the implied embedding size would be larger than the original vocabulary. In each remaining bin, we perform a grid search of $\embsize$ to find the minimum value that yields $r@100 = 0.95$ for the bin. As shown in \autoref{fig:treccar-query-recall-at-100}, the relationship between $\embsize$ and the theoretical quantity $(\epsilon^2/2 - \epsilon^3/3)^{-1}$ is roughly linear, showing that the theory is applicable to \bm ranking. 
\begin{figure}
    % see //experimental/users/jeisenstein/text_vectors/make_rademacher_query_fig.py
    % https://cnsviewer2.corp.google.com/cns/lu-d/home/lumiere/public/data/vectors/tacl_figures/treccar_query_recall_10.pdf
    \centering
    \includegraphics[width=\linewidth]{figures/treccar_query_rank=100_bins=50_err=05_novac_cubic.pdf}
    \caption{Relationship between the minimum normalized margin $\epsilon$ and the minimum embedding size that achieves recall@100=0.95 for the \treccar dataset. Each point corresponds to a group of queries, binned by the normalized margin $\nmarg(q, d_1, d_{100})$, as described in the text. \mike{I think the older figure was perhaps better. Excluding points where the bound is vacuous because the constants could be very pessimistic. Could we plot the old figure and show the linear relationship, with the exception of the single outlier point? We could then argue that the relationship is close to that predicted by the bound except for extreme points.}}
    \label{fig:treccar-query-recall-at-100}
\end{figure}
}


==> tables/rerank_by_step.tex <==
 \begin{table}[!t]
   \centering
   \small
   \scalebox{.75}{
   % fussily removed vertical lines, feel free to add back if you feel strongly about it -J
   \begin{tabular}{l @{\hspace{0.1cm}} c  c  c  c c c c}
     \toprule
     \multirow{2}{*}{Retriever} & \multicolumn{7}{c}{Depth } \\
     \cmidrule{2-8}
      & {10} & {20} & {50} & {100} & {200} & {500} & {1000}\\
      \midrule
   \multicolumn{8}{c}{MS MARCO passage} \\
   \midrule
   \textsc{DeepCT} & 0.320  & 0.343  & 0.361  & 0.368 & 0.370 & 0.374 & 0.376 \\
   BM25 & 0.256 & 0.292 & 0.326 & 0.346 & 0.361 & 0.374 & 0.376\\
  DE-BERT & 0.356 & 0.369 & 0.381 & 0.387 & 0.389 & 0.390 & 0.391 \\
   ME-BERT & 0.374 & 0.383 & 0.389 & 0.393 & 0.394 & 0.394 & 0.395 \\
     \textsc{hybrid} & 0.371 & 0.381 & 0.387 & 0.389 & 0.390 & 0.390 & 0.390 \\
   \midrule
      \multicolumn{8}{c}{MS MARCO document} \\
   \midrule

BM25 & 0.292 & 0.318 & 0.330 & 0.337 & 0.337 & 0.334 & 0.334 \\
DE-BERT & 0.297 & 0.315 & 0.326 & 0.330 & 0.336 & 0.338 & 0.339 \\
ME-BERT & 0.333 & 0.344 & 0.352 & 0.353 & 0.353 & 0.352 & 0.353 \\
     \textsc{hybrid} & 0.342 & 0.354 & 0.357 & 0.354 & 0.354 & 0.353 & 0.353 \\

     \bottomrule
   \end{tabular}
   }
   \caption{{\small{MRR@10 when reranking at different depth for the MS MARCO passage and document tasks. }}}
   \label{tab:msmarco_depth}
\end{table}


